Occlusion Sensitivity Analysis with Augmentation Subspace Perturbation in Deep Feature Space

Deep Learning of neural networks has gained prominence in multiple life-critical applications like medical diagnoses and autonomous vehicle accident investigations. However, concerns about model transparency and biases persist. Explainable methods are viewed as the solution to address these challenges. In this study, we introduce the Occlusion Sensitivity Analysis with Deep Feature Augmentation Subspace (OSA-DAS), a novel perturbation-based interpretability approach for computer vision. While traditional perturbation methods make only use of occlusions to explain the model predictions, OSA-DAS extends standard occlusion sensitivity analysis by enabling the integration with diverse image augmentations. Distinctly, our method utilizes the output vector of a DNN to build low-dimensional subspaces within the deep feature vector space, offering a more precise explanation of the model prediction. The structural similarity between these subspaces encompasses the influence of diverse augmentations and occlusions. We test extensively on the ImageNet-1k, and our class- and model-agnostic approach outperforms commonly used interpreters, setting it apart in the realm of explainable AI.

==> sections/background.tex <==

In this section we skim over the theoretical background of our approach. Given the space limits, we do not present the full framework, but instead informally discuss the intuition behind. Details can be found in the supplementary material.

\subsection{Explanations}

An explanation in the context of machine learning models is a map describing how the model's predictions are influenced by each of the input variables. It seeks to identify which portions of the input (\eg, pixels in an image) are most responsible for a given output. Each entry in the explanation heatmap is a measurement of the degree of responsibility of the respective entry in the input to the model prediction, similar to a binary instance segmentation output.

More formally, Let $f$ be a machine learning model and $x$ an input with output $f(x)$, and $S = x \odot M$ a masked subset of the input. Then, the explanation $E$ is 

\begin{equation}
    E(f|x) = \min_{|S|} S : f(S) = f(x), |S| > 0
\end{equation}

However, computing an explanation is NP-complete and real interpreters will output approximate explanations~\cite{chockler_explanations_2021}. These approximations mean that the real explanation heatmaps will be probability distributions indicating if the input entry belongs to the actual cause of prediction.

\subsubsection{Minimal Size Metric}

The approximate explanation leads us to think of metric for how close the explanation heatmap is to the actual cause. The minimal size of the cause of the prediction is the ratio between the minimal number of pixels which maintains the prediction and the original number of pixels in the image.

\begin{equation}
    s_{min}(E(f|x)) = \frac{|S|}{|x|}, f(S) = f(x)
\end{equation}

In practical terms, this could be measured by keeping only a percentile of the image pixels following the ascending order of degree of responsibility according to the heatmap $E$. Thus, when comparing interpreters, the lower the minimal size, the better because it means the approximate explanation should be closer to the actual cause.

\subsection{Subspace Analysis}

This section offers an introduction to subspace representation, elaborates on the core concept, and introduces canonical angles, providing a comprehensive understanding of the topic.

Subspace analysis in computer vision encompasses a framework that facilitates comparison and classification of various subspaces. Core techniques in this domain are the subspace method (SM) and Mutual Subspace method (MSM), which uses cosine similarity as a measure of subspace distance. Each subspace encapsulates the distribution of pattern vectors in a high-dimensional vector space \cite{fukui_difference_2015}.

\subsubsection{Subspace Representation}

A subspace \( \mathcal{P} \) of a larger vector space $U$ is represented as an orthonormal basis $\mathbf{P}$ of the set of vectors $x_i$ that form \( \mathcal{P} \). Concretely, the basis matrix $\mathbf{P} = \{\mathbf{p}_0,\mathbf{p}_1,\dots,\mathbf{p}_n\}$ can be obtained by applying Principal Component Analysis (PCA) to the correlation matrix $\sum x_i x_i^T$.

% \begin{equation}
%     \mathbf{P} = PCA(\sum x_i x_i^T)
% \end{equation}

\subsubsection{Canonical Angles}

Given two subspaces \( \mathcal{P} \) and \( \mathcal{Q} \), the canonical angles $\theta_i$ between the two subspaces are defined as the lowest angles between two pairs of vectors of their respective basis vectors $\mathbf{p}_i$ and $\mathbf{q}_i$

\begin{equation}
    \cos^2\theta_i = \max_{\substack{\mathbf{p}_i \perp \mathbf{q}_i \\ \mathbf{p}_i \perp \mathbf{q}_i}} \frac{(\mathbf{p}_i \cdot \mathbf{q}_i)^2}{||\mathbf{p}_i||^2 ||\mathbf{q}_i||^2}
\end{equation}

However, a more practical method to obtain the canonical angles is to compute the singular values of the product of basis matrices~\cite{fukui_subspace_2020}.

\subsubsection{Subspace Similarity}

The canonical angles are used to define a measurement of structural similarity $Sim$ between subspaces~\cite{fukui_subspace_2020}. The subspace similarity thus is defined as the sum of the $D$ smallest canonical angles, where $D$ is a hyperparameter which indicates how much information from each subspace is to be considered.

\begin{equation}
    Sim(\mathcal{P}, \mathcal{Q}) = \sum_i^D \cos^2\theta_i 
\end{equation}

Alternatively, the orthogonal degree is a measurement of subspace divergence~\cite{fukui_difference_2015}, \ie, how different the subspaces are, and can be defined as $1 - Sim(\mathcal{P}, \mathcal{Q})$.


